Probing lepton number violating interactions in rare kaon decays

We investigate the possibility to probe lepton number violating (LNV) operators in the rare kaon decay $K\to\pi\nu\nu$. Performing the analysis in the Standard Model effective field theory with only light active Majorana neutrinos, we determine the current limits on the corresponding LNV physics scale from the past E949 experiment at BNL as well as the currently operating experiments NA62 at CERN and KOTO at J-PARC. We focus on the specific signature of scalar currents in $K\to\pi\nu\nu$ arising from the LNV nature of the operators and study the effect on the experimental sensitivity, stressing the need for dedicated searches for beyond the SM currents. We find that the rare kaon decays probe high operator scales $\Lambda_\text{LNV} \approx 15$ to $20$ TeV in different quark and neutrino flavours compared to neutrinoless double beta decay. Furthermore, we comment that the observation of LNV in kaon decays can put high-scale leptogenesis under tension. Finally, we discuss the connection with small radiatively generated neutrino masses and show how the severe constraints therefrom can be evaded in a minimal ultraviolet-complete scenario featuring leptoquarks.

==> leptogenesis.tex <==
\subsection{Leptogenesis}\label{leptogenesis}

In order to generate the observed baryon asymmetry, any LNV process cannot be too effective in the early universe, as it could then wash out the asymmetry via sphalerons. In this section, we estimate the energy scale $\lambda$ at which the washout stops being effective, for the operators in the previous sections, following the method used in \cite{Deppisch:2018}. The dynamics of the lepton number for a given operator is described by the Boltzmann equation \cite{Buchmuller:2005}
%
\begin{equation}
\label{eq:Boltzmann}
    zHn_{\gamma}\frac{d\eta_{L}}{dz} = -\lr{\frac{n_{i}n_{j}\dots}{n^{\text{eq}}_{i}n^{\text{eq}}_{j}\dots} - \frac{n_{\bar{k}}n_{\bar{l}}\dots}{n^{\text{eq}}_{\bar{H}}n^{\text{eq}}_{\bar{Q}}\dots}}\gamma^{\text{eq}}\lr{ij\dots \rightarrow  \bar{k}\bar{l}\dots} + \text{permutations.}
\end{equation}
%
Here, $n_i$ is the number density of particle $i$, with $\eta_i \equiv n_i/n_\gamma$, and where $n_\gamma$ is the number density of photons. Furthermore, $H$ is the Hubble constant, and $z$ has the dimension of inverse temperature. A superscript \textit{eq} means at equilibrium, and $\gamma^{\text{eq}}$ denotes the equilibrium reaction density. The dots represent any other particle species, or multiplet of species, that is included in the operator at hand, and by \textit{permutations} is meant all other possible orderings of the fields in the operator (including the Hermitian conjugate) that contain at least two particles in either initial or final state. The reaction density can be estimated as \cite{Giudice:2004}
%
\begin{equation}
\label{eq:scatterdens}
    \gamma^{\text{eq}} = \frac{2^{2(n_f + m_f) - 2}}{(2\pi)^{2(n + m) - 3}}\frac{1}{n^{n_f}m^{m_f}}\frac{\Gamma\lr{D - 3}\Gamma\lr{D - 2}}{\Gamma\lr{n}\Gamma\lr{n - 1}\Gamma\lr{m}\Gamma\lr{m - 1}}\frac{T^{2D - 4}}{\Lambda^{2D - 8}}.
\end{equation}
%
Here, $n$ ($m$) denotes the number of initial (final) particles, where a subscript $f$ counts only the fermions. Furthermore, $D$ is the dimension of the operator, $\Lambda$ is the NP scale, $T$ is the temperature and $\Gamma$ is the gamma function. The number densities in Eq.~\eqref{eq:Boltzmann} can be estimated using chemical potentials \cite{Harvey:1990},
%
\begin{equation}
\label{eq:chempot}
    \frac{n_i}{n^{\text{eq}}_i} \approx e^{\mu_i/T} \approx 1 + \frac{\mu}{T}.
\end{equation}
%
Here, $\mu_i$ is the chemical potential of particle species $i$, which has the opposite sign for the anti-particle. The chemical potentials of the different fields of the SM can be related to each other by assuming that the SM Yukawa interactions, as well as the sphaleron process, are in equilibrium, and the different chemical potentials can in this way all be expressed in terms of the lepton doublet chemical potential \cite{Harvey:1990}. Having used Eqs.~\eqref{eq:scatterdens} and \eqref{eq:chempot} in the Boltzmann equation, it can be expressed as
%
\begin{equation}
    \label{eq:secondBoltzmann}
    \frac{d\eta_{\Delta L}}{dz} = - \frac{\eta_{\Delta L}}{z}c'_D\frac{\Lambda_{\text{pl}}}{\Lambda}\lr{\frac{T}{\Lambda}}^{2D-9},
\end{equation}
%
where $\eta_{\Delta L} \equiv \eta_L - \bar{\eta}_L$, the dimensionless coefficient $c_D'$ is determined by relating the different chemical potentials as previously described, and
%
\begin{equation}
	\Lambda_{\text{pl}} = \sqrt{\frac{8\pi^3}{90}}\frac{\sqrt{g_*}T^2}{H}
\end{equation}
%
is the Planck scale, assuming a flat Friedmann-Robertson-Walker universe, where $g_*$ is the number of relativistic degrees of freedom in the SM. Solving the Boltzmann equation in Eq.~\eqref{eq:secondBoltzmann} gives \cite{Buchmuller:2005}
%
\begin{equation}
\label{eq:Boltzmannsolution}
    \ln\lr{\frac{\eta_{\Delta L\text{,EW}}}{\eta_{\Delta L\text{,B}}}} = \frac{c'_D}{(2D - 9)}\frac{\Lambda_{\text{pl}}}{\Lambda^{2D - 8}}\lr{\frac{1}{z_{\text{EW}}^{2D - 9}} - \frac{1}{z_{\text{B}}^{2D - 9}}}.
\end{equation}
%
Here, a subscript B means that the variable is obtained at the baryogenesis scale, while EW corresponds to the scale of electroweak symmetry breaking $v = 176$ GeV. The lepton asymmetry at the electroweak scale has to correspond to the observed baryon asymmetry, assuming there is no LNV process below this energy. Solving Eq.~\ref{eq:Boltzmannsolution} for the temperature corresponding to $z_B$ then gives the energy scale $\lambda$ at which the washout effectively stops. This washout scale is shown in Table~\ref{tab:d7mesondecay2}, and it is very close to the electroweak symmetry breaking scale for all listed LNV observables at their current experimental limits. Taking the NP scale as the upper limit for the washout for each operator, we have a range over which the washout is effective. The observation that the washout is effective over a wide energy range for all dimension-7 operators in the meson decays tells us that any NP in these rare decays would reveal a new contribution to the washout in a leptogenesis scenario.


==> newcommands.tex <==
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\ddx}[1]{\frac{d #1}{dx}}
\newcommand{\dpdp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dirac}[2]{\delta^{(3)}(\mathbf{#1}-\mathbf{#2})}
\newcommand{\vt}{\vec{v}^{\bot}}
\newcommand{\sn}{\vec{S}_{N}^{\,r'r}}
\newcommand{\sx}{\vec{S}_{\chi}^{\,s's}}
\newcommand{\sX}{\vec{S}_{X}^{\,s's}}
\newcommand{\sndag}{\vec{S}_{N}^{\,rr'}}
\newcommand{\sxdag}{\vec{S}_{\chi}^{\,ss'}}
\newcommand{\sXdag}{\vec{S}_{X}^{\,ss'}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\Op}{\mathcal{O}}
\newcommand{\Sy}{\mathcal{S}}
\newcommand{\qmn}{\tfrac{\vec{q}}{m_N}}
\newcommand{\es}{\vec{e}_s}
\newcommand{\esp}{\vec{e}\,'_{s'}}
\newcommand{\lvector}[2]{\begin{pmatrix}
#1\\
#2
\end{pmatrix}}
\newcommand{\hvector}[2]{\begin{pmatrix}
#1\! & #2
\end{pmatrix}}
\newcommand{\twomatrix}[4]{\begin{pmatrix}
#1 & #2\\
#3 & #4\
\end{pmatrix}}
\newcommand{\iM}{i\mathcal{M}}
\newcommand{\iMb}{i\bar{\mathcal{M}}}
\newcommand{\sw}{\sin^2\theta_W}
\newcommand{\pl}{\left(1 - \gamma_5\right)}
\newcommand{\pr}{\left(1 + \gamma_5\right)}
\newcommand{\prl}{\left(1 \pm \gamma_5\right)}
\newcommand{\tenr}{\frac{i}{2}\left[\gamma^\mu,\gamma^\nu\right]}
\newcommand{\hc}{\text{h.c}}
\newcommand{\lr}[1]{\left(#1\right)}
\newcommand{\new}{\text{ \textcolor{red}{New!}}}


\def\Julia#1{{\bf  \textcolor{BrickRed}{[Julia: {#1}]}}}
\def\Kare#1{{\bf  \textcolor{BurntOrange}{[K\r{a}re: {#1}]}}}
\def\Frank#1{{\bf  \textcolor{magenta}{[Frank: {#1}]}}} 

